Learning Deep Features in Instrumental Variable Regression

Instrumental variable (IV) regression is a standard strategy for learning causal relationships between confounded treatment and outcome variables from observational data by utilizing an instrumental variable, which affects the outcome only through the treatment. In classical IV regression, learning proceeds in two stages: stage 1 performs linear regression from the instrument to the treatment; and stage 2 performs linear regression from the treatment to the outcome, conditioned on the instrument. We propose a novel method, deep feature instrumental variable regression (DFIV), to address the case where relations between instruments, treatments, and outcomes may be nonlinear. In this case, deep neural nets are trained to define informative nonlinear features on the instruments and treatments. We propose an alternating training regime for these features to ensure good end-to-end performance when composing stages 1 and 2, thus obtaining highly flexible feature maps in a computationally efficient manner. DFIV outperforms recent state-of-the-art methods on challenging IV benchmarks, including settings involving high dimensional image data. DFIV also exhibits competitive performance in off-policy policy evaluation for reinforcement learning, which can be understood as an IV regression task.

==> Experiment/ope_org.tex <==

Consider a Markov decision process of state space $\mathcal{S}$, action space $\mathcal{A}$, and discount factor $\gamma \in [0,1)$  where $p(s'|s,a)$ denotes the probability of making a transition to state $s'$ when taking action $a$ in state $s$ while $\mu(r|s,a,s')$ denotes the probability density of reward $r$ when having moved to $s'$ from $s$ after having taken action $a$. For the policy $\pi$ where $\pi(a|s)$ denotes the probability of taking action $a$ in state $s$, the Q-function is given by

\begin{equation}
    Q(s,a)=\mathbb{E}\left[\sum_{t=0}^\infty \gamma^t r_t | s_0=s, a_0=a\right],
\end{equation}
where the expectation is w.r.t.
\begin{equation}
    \prod_{t=1}^\infty p(s_t|s_{t-1},a_{t-1})\mu(r_{t}|s_{t-1},a_{t-1},s_{t})\pi(a_t|s_t).
\end{equation}
This Q-function satisfies the following Bellman equation
\begin{equation}\label{eq:BellmanQ}
    Q(s,a)=R(s,a)+\gamma \int\int p(s'|s,a)\pi(s'|a') Q(s',a')\textrm{d}s'\textrm{d}a',
\end{equation}
where the average reward is given by
\begin{equation}
    R(s,a)=\int r~p(s'|s,a)\mu(r|s,a,s') \textrm{d}r \textrm{d}s'.
\end{equation}
We typically cannot compute in closed-form the Q-function as we can only sample from $p(s'|s,a)$ and $\mu(r|s,a,s')$ but do not have access to their expressions. However, when we have access to tuples of the form $(s_t,a_t,r_t,s_{t+1})$ having been obtained using any policy, we will show that, for any policy $\pi$, we can obtain a neural network approximation of the $Q$ function using IV regression. This generalizes the Least Squares Temporal Difference (LSTD) approach of \cite{bradtke1996linear} which uses the standard 2SLS method to approximate a linearly parameterized value function.

The key is to rewrite (\ref{eq:BellmanQ}) using the following decomposition
\begin{align}
    r&=Q(s,a)-\gamma Q(s',a')\nonumber\\
    &+\gamma\left(Q(s',a') - \int p(s'|s_t,a_t)\pi(a'|s')Q(s',a')ds'da'\right)\nonumber\\
    &+r-R(s,a).\label{eq:Keydecomposition}
\end{align}
This can be rewritten as a structural causal model \eqref{eq:structuralcausalmodel} where $Y=r$ is the outcome, $X=(s,a,s',a')$ the treatment and $Z=(s,a)$ the instrument while the structural function is 
\begin{align*}
      f_\mathrm{str}(a,s,a',s')=Q(a,s)-\gamma Q(a',s') 
\end{align*}
and the confounder $\varepsilon$ is
\begin{align}\label{eq:Noise}
    \varepsilon&=\gamma\left(Q(s',a') - \int p(s'|s_t,a_t)\pi(a'|s')Q(s',a')ds'da'\right)\nonumber\\
    &+r_t-R(s,a),\nonumber\\
\end{align}
which is indeed such that $\expect{\varepsilon}= 0$, $\expect{\varepsilon | X}\neq 0$ if, for any available tuple $(s,a,r,s')=(s_t,a_t,r_t,s_{t+1})$, we sample $a'=a_{t+1}\sim \pi(a'|s')$. We also have $\expect{\varepsilon | Z}=0$ as required.

In this context, we want here to model $Q(s,a)=\vec{f}^\top \vec{\psi}_{\theta_X}(s,a)$ so 
\begin{align}\label{eq:SCMforQ}
    f_\mathrm{str}(s,a,s',a') = \vec{f}^\top (\vec{\psi}_{\theta_X}(s,a) - \gamma \vec{\psi}_{\theta_X}(s',a')).
\end{align}
It follows that 
\begin{align*}
\expect[X|z]{f(X)} = \vec{f}^\top(\vec{\psi}_{\theta_X}(s,a)- \gamma \expect[s',a'|s,a]{\vec{\psi}(s',a')}).
\end{align*}
We will model $\expect[s',a'|s,a]{\vec{\psi}(s',a')}=E \vec{\phi}(s,a)$.
In this case, given data $(s_t,a_t,s_{t+1},a_{t+1})$, stage 1 is not modified and requires solving 
\begin{align}
    \hat{E}^{(m)}, \hat{\theta}_Z = \argmin_{E \in \mathbb{R}^{d_1 \times d_2}, \theta_Z} \mathcal{L}_1^{(m)}, \quad \mathcal{L}_1^{(m)} = \frac1m \sum_{t=1}^m \|\vec{\psi}_{\theta_X}(s_t,a_t) - E\vec{\phi}_{\theta_Z}(s_{t+1},a_{t+1})\|^2 + \lambda_1 \|E\|^2. \label{eq:stage1-empirical-loss_Q}
\end{align}
However, given the specific form \eqref{eq:SCMforQ} of the structural function, stage 2 is slightly modified and requires minimizing for data $(r_t,s_t,a_t)$ the loss
\begin{align}
    \hat{\vec{f}}^{(n)}, \hat{\theta}_X = \argmin_{\vec{f} \in \mathbb{R}^{d_1}, \theta_X}\mathcal{L}^{(n)}_2, \quad \mathcal{L}^{(n)}_2 = \frac1n \sum_{t=1}^n (r_t - \vec{f}^\top (\vec{\psi}_{\theta_X}(s_t,a_t)-\gamma\hat{E}^{(m)} \vec{\phi}_{\theta_Z}(s_t,a_t)))^2 + \lambda_2 \|\vec{f}\|^2. \label{eq:stage2-empirical-loss_Q}
\end{align}

==> Introduction/related_work.tex <==
Several approaches have been proposed for non-linear IV regression. One approach is 
to correct the bias caused by the hidden confounder by estimating the conditional distribution of the treatment given the instrumental. The first literature take this approach are \citet{Carrasco2007, Darolles2011}, in which the conditional distribution is estimated by a ratio of Nadaraya-Watson density estimates. One advantage of this approach is that it allows us to learn arbitrary flexible models. In DeepIV \citep{Hartford2017}, the structural function is modeled by deep neural networks and the density is also estimated via mixture density networks \citep{Bishop2006}. Despite the rich expressiveness of the model, the learning tends to be unstable, especially when the treatment is high-dimensional, due to ``forbidden regression'' issue.

Another approach is to extend the 2SLS algorithm based on non-linear basis functions. The first literature taking this approach is sieve IV \citep{Newey2003, Chen2018}, which uses a finite number of basis functions explicitly specified. KIV (kernel instrumental variable regression) \citep{Singh2019} extends sieve IV to allow for an infinite number of basis functions using RKHS. Although these methods enjoy good theoretical properties, the complexity of models can be limited, since they use prespecified basis functions. Our method, DFIV, utilizes this approach but adaptively learns flexible basis functions from data. 

The third approach is to use the generalized method of moment (GMM) \citep{Hansen1982} to find a structural function so that the residual and the instrumental is independent. Recently, \citet{Bennett2019} proposes DeepGMM, which solves a variational formulation of GMM within a highly flexible function space. Although this approach can handle high-dimensional treatment variable, the learning might not be as stable as 2SLS approach, since it involves solving a smooth zero-sum game.


==> Method/adaptive_feature.tex <==
Let us consider the supervised learning setting, which aims to learn a feedforward neural net $y$ predicting $Y$ from $X$ given data ${(x_i, y_i)}$. Assume that the final layer of $y$ is a linear layer, i.e. $y(x) = \vec{w}^\top \vec{h}_\theta(x)$ with weight vector $\vec{w} \in \mathbb{R}^{d_w}$ and network activations $\vec{h}_\theta$ parameterised by $\theta$. Now, we minimize the following mean-squared error with $\ell_2$-regularization
\begin{align*}
    \hat{\vec{w}}, \hat{\theta} = \argmin_{\vec{w}, \theta} \mathcal{L}(\vec{w}, \theta), \quad \mathcal{L}(\vec{w}, \theta)= \sum_{i=1}^n \|y_i - \vec{w}^\top \vec{h}_\theta(x_i)\|^2 + \lambda\|\vec{w}\|^2 + \lambda\|\theta\|^2 
\end{align*}
to learn the parameters $\hat{\vec{w}}, \hat{\theta}$. The standard way of optimizing this is by gradient descent, where the estimates $\hat{\vec{w}}_t$ and $\hat{\theta}_t$ at iteration $t$
are updated using
\begin{align}
    \hat{\vec{w}}_{t+1} \leftarrow \hat{\vec{w}}_{t} - \nabla_{\vec{w}}  \mathcal{L}(\hat{\vec{w}}_{t}, \hat{\theta}_t), \quad \hat{\theta}_{t+1} \leftarrow \hat{\theta}_{t} - \nabla_{\theta}  \mathcal{L}(\hat{\vec{w}}_t, \hat{\theta}_{t}). \label{eq:joint-gradient-descent}
\end{align}
Instead, we first solve the minimization problem for $\vec{w}$ with $\theta$ fixed to $\hat{\theta}_t$, and then, take a gradient step for $\theta$ while $\vec{w}$ is fixed to $\hat{\vec{w}}_t$. That is,
%Since the minimizing argument $\hat{\vec{w}}_t$ can be explicitly computed via the linear ridge regression formula, the update is given as follows
\begin{align}
    \hat{\vec{w}}_{t} \leftarrow \left(H_t^\top H_t + \lambda I\right)^{-1}\left(H_t^\top \vec{y}\right), \quad 
    \hat{\theta}_{t+1} \leftarrow \hat{\theta}_{t} - \nabla_{\theta}\mathcal{L}(\hat{\vec{w}}_{t}, \hat{\theta}_{t}), \label{eq:learn-adaptive-feature}
\end{align}
where $H_t = [\vec{h}_{\hat{\theta}_t}(x_1), \dots, \vec{h}_{\hat{\theta}_t}(x_n)]^\top \in \mathbb{R}^{n\times d_w}$ and  $\vec{y} = [y_1, \dots, y_n]^\top$.
\yccomment{Do we treat $\hat{\vec{w}}$ as a function of $\theta$ and back-propagate the gradient of $\mathcal{L}$ through it? I think this is what we do in the implementation. There's a big difference from the current presentation. Current Eq.~\ref{eq:learn-adaptive-feature} is a kind of semi-coordinate descent.}
The approach in \eqref{eq:learn-adaptive-feature} can converge faster to a good solution compared to the approach in \eqref{eq:joint-gradient-descent}, as shown in Appendix~\ref{sec:learning-comparison}. Furthermore, this will enable us to back-propagate the loss of stage 2 to the feature map of the treatment variable in the 2SLS algorithm.




==> Method/hyper-param.tex <==
If observations from the joint distribution of $(X, Y, Z)$ are available in both stages, we can tune the regularization parameters $\lambda_1, \lambda_2$ using the approach proposed in \citet{Singh2019}. Let the complete data of stage 1 and stage 2 be denoted as $(x_i, y_i, z_i)$ and $(\tilde x_i, \tilde y_i, \tilde z_i)$. Then, we can use the data not used in each stage to evaluate the out-of-sample performance of the other stage. Specifically, the regularizing parameters are given by
\begin{align*}
    &\lambda_1^* = \argmin \mathcal{L}_{1\text{-oos}}^{(n)}, \quad \mathcal{L}_{1\text{-oos}}^{(n)} = \frac1n \sum_{j=1}^n \|\vec{\psi}_{\hat\theta_X}(\tilde x_i) - \hat{\vec{V}}^{(m)}\vec{\phi}_{\hat\theta_Z}(\tilde z_i)\|^2,\\
    &\lambda_2^* = \argmin \mathcal{L}_{2\text{-oos}}^{(n)}, \quad\mathcal{L}_{2\text{-oos}}^{(n)} = \frac1m \sum_{i=1}^m (y_i - (\hat{\vec{u}}^{(n)})^\top \hat{\vec{V}}^{(m)} \vec{\phi}_{\hat\theta_Z}(z_i))^2,
\end{align*}
where $\hat{\vec{u}}^{(n)}, \hat{\vec{V}}^{(m)}, \hat{\theta}_{\theta_X}, \hat{\theta}_{\theta_Z}$ are the parameters learned in \eqref{eq:stage1-empirical-loss} and \eqref{eq:stage2-empirical-loss}.


==> Method/method_intro.tex <==
In this section, we formulate our proposed method, {\it deep feature instrumental variable regression} (DFIV).% We first introduce an approach to learn adaptive features in the standard supervised setting, and then apply it to construct our two-stage DFIV algorithm. 

==> junk_piece/deep_kernel.tex <==
In DFIV, we learn the adaptive basis functions. Let $\vec{\psi}_{\theta_X}(x): \mathcal{X} \to \mathbb{R}^{d_1}$ and $\vec{\phi}_{\theta_Z}(z):\mathcal{Z} \to \mathbb{R}^{d_2}$ are the basis functions that are parameterized by $\theta_X$ and $\theta_Z$, respectively. We do not put any further assumption on these feature maps, except parameters can be learned from gradient descent method. Given these functions, we define the model
\begin{align*}
    f_\mathrm{str}(x) = \vec{f}^\top \vec{\psi}_{\theta_X}(x), \quad \expect[X|z]{\vec{\psi}_{\theta_X}(X)} = E\vec{\phi}_{\theta_Z}(z),
\end{align*}
where parameters $\vec{f}, E, \theta_X, \theta_Z$ are tuned during the training.

From the perspective from kernel methods, using this feature map corresponds to consider the kernel functions $k_\mathcal{X}: \mathcal{X}\times\mathcal{X} \to \mathbb{R}$ and $k_\mathcal{Z}: \mathcal{Z}\times\mathcal{Z} \to \mathbb{R}$ defined as
\begin{align}
    k_\mathcal{X}(x, x') = (\vec{\psi}_{\theta_X}(x))^\top \vec{\psi}_{\theta_X}(x') \quad k_\mathcal{Z}(z, z') = (\vec{\phi}_{\theta_Z}(z))^\top \vec{\phi}_{\theta_Z}(z'). \label{eq:kernel-def}
\end{align}

In the most of literature on deep kernels\adcomment{add relevant refs}, we try to learn kernel functions formulated as $k(x,x') = \kappa(\psi(x), \psi(x'))$ where $\kappa$ is a static positive definite kernel and $\psi$ is a neural network. Hence, our kernel function \eqref{eq:kernel-def} can be regarded as the simplest type of such deep kernels, in which $\kappa$ corresponds to the inner product of Euclidean space.

In general, kernel ridge regression requires to compute the inverse of the Gram matrix which takes a time cubic in the data size. However, if we use the kernel \eqref{eq:kernel-def}, all we have to do is linear regression based on the features $\vec{\psi}_{\theta_X}, \vec{\phi}_{\theta_Z}$, which greatly reduces the computational complexity, yet still makes use of the flexibility of neural networks. We will discuss the computational complexity in detail after introducing the algorithm.

==> junk_piece/demand_data_generation.tex <==
\subsection{Data Generating Process} 

We used the synthetic data that models the problem of predicting the demand for the airline tickets. It is assumed that there are 7 customer types $s \in \{1,...,7\}$ that each exhibit different levels of price sensitivity. Given the price $p$ and the time of year $t$, the structure function we aim to learn is 
\begin{align*}
    &f_{\text{str}}(p, t, s) = 100 + (10 + p) \cdot s \cdot \eta(t) + 2p.
    %&\psi(t) = 2\left((t-5)^4/600+\exp\left(-4(t-5)^2\right)+t/10-2\right)
\end{align*} 
Here, $\eta(t)$ is a complex function, which reflects the high demand in the holiday season. We sample time of year $t$ from $t\sim \mathrm{Unif}(0, 10)$ and select customer type $s$ uniformly from $\{1,\dots,7\}$ to build training data. The price $p$ is determined from the fuel price $c$ and the time of the year $t$ as $p=25+(c+3)\eta(t) + \nu$, where $\nu$ is a additive noise.

The observed demand $y$ is given by the $y = f_\mathrm{str}(p,t,s) + \varepsilon$ where $\varepsilon$ is an additive noise that is correlated with the noise in price $\nu$. This correlation reflects the fact that the price and demand are both cofounded by supply-side market forces. Parameter $\rho$ determines correlation between $\varepsilon$ and $\nu$, and we report the result of the various value of $\rho =\{0.9, 0.75, 0.5, 0.25,0.1\}$. As in \citet{Singh2019,Hartford2017}, the performance is evaluated by the mean squared error from $f_\mathrm{str}$, where the test points are uniformly sampled from space of $(p,t,s)$. This requires the model to successfully extrapolate the prediction, which is discussed in Appendix~\ref{sec:cov_shift}.



==> junk_piece/high_dim.tex <==
In high-dimensional setting, we use the same treatment variable $X=(p, t, s)$ and $Z = (c, t, s)$, but the customer type label $s \in \{1,\dots,7\}$ is replaced with the image of the corresponding handwritten digit from the MNIST dataset \citep{mnist}. This reflects the fact that we cannot know the exact customer type and thus we need to estimate it from high-dimensional data. Although the task itself has not changed, this problem becomes far more difficult than the low-dimensional case. 

Here, we used the same architecture as in the low-dimensional setting with adding one fully-connected layer to extract the feature from the image. Note that this is a significantly simpler network compared to DeepIV. We set hyper-parameter in the way discussed in Appendix~\ref{sec:hyper}. We ran 20 simulations with data size $n+m=5000$, and the mean and the variance of MSE is shown in Table~\ref{table:high-dim}. 

\begin{table}[t]
  \caption{MSE for high dimensional domain. The bold face means
        the outstanding method chosen by Welch t-test with the significance level 5\%}
      \begin{tabular}{l@{\hspace{3pt}}ccccc} \toprule
         & $\rho=0.9$ & $\rho=0.75$ & $\rho=0.5$ & $\rho=0.25$ & $\rho=0.1$ \\\midrule
         DFIV &  {\bf 10741 (1747)} & {\bf  10734 (1509)} & {\bf 10912 (1697)} & {\bf  11705 (2163)} & {\bf 10728 (1483)}\\
          DFIV (vanilla) & 14733 (2449) &   14372 (2827) & 12421 (2293) & 13610 (2110) & 13871 (2134)\\ %without normalization
        DeepIV &14224 (646)&14301 (719)&14473 (833)&14207 (633)&14189 (725)\\
        
        KIV&21161 (1134)&21162 (1134)& 21164 (1134)&21164 (1134)&21164 (1133)\\
        \bottomrule
      \end{tabular}
      \label{table:high-dim}
  \end{table}

  In the high-dimensional setting, KIV is suffered from the curse of dimension, which significantly harms the performance. Moreover, we observe vanilla DFIV performs as good as DeepIV in spite of its small network, which also suggests the superiority of the method. Finally, we can further improve the performance by applying the Spectral Normalization.

==> junk_piece/junk_appendices/feature_map_learning.tex <==
Here, we compare the approach of learning the adaptive feature maps to the learning the ordinary feed-forward network. Let consider the following regression problem.
\begin{align*}
    \hat{\vec{f}}, \hat{\theta} = \argmin_{\vec{f}, \theta} \mathcal{L}(\vec{f}, \theta), \quad \mathcal{L}(\vec{f}, \theta)= \sum_{i=1}^n \|y_i^2 - \vec{f}^\top \vec{\phi}_\theta(x_i)\|^2 + \lambda\|\vec{f}\|^2,
\end{align*}
where $(x_i, y_i)$ are data, and $\vec{\phi}_\theta$ denotes the adaptive feature map parmameterized by $\theta$. If we use simple feedforward neural network, this is learned by jointly update $\vec{f}$ and $\theta$ using gradient-decent methods.
\begin{align*}
    \hat{\vec{f}}_{t+1} \leftarrow \hat{\vec{f}}_{t} - \nabla_{\vec{f}}  \mathcal{L}(\vec{f}, \hat{\theta}_t), \quad \hat{\theta}_{t+1} \leftarrow \hat{\theta}_{t} - \nabla_{\theta}  \mathcal{L}(\hat{\vec{f}}_t, \theta),
\end{align*}
where $\hat{\vec{f}}_t$ and $\hat{\theta}_t$ are the estimation of $\hat{\vec{f}}$ and $\hat{\theta}$ at $t$-th epoch, respectively.
Let us call this approach as {\tt Joint-Gradient-Descent}. The approach we used is to first solve the minimization problem to get $\hat{\vec{f}}$ fixing $\theta$. Then, take a gradient step for $\vec{f} = \hat{\vec{f}}_t$.
\begin{align*}
    \hat{\vec{f}}_{t+1} \leftarrow \left(\Phi_t^\top \Phi_t + \lambda I\right)^{-1}\left(\Phi_t^\top \vec{y}\right), \quad 
    \hat{\theta}_{t+1} \leftarrow \hat{\theta}_{t} - \nabla_{\theta}\mathcal{L}(\hat{\vec{f}}_{t+1},\theta)
\end{align*}
where $\Phi_t = [\vec{\phi}_{\hat{\theta}_t}(x_1), \dots, \vec{\phi}_{\hat{\theta}_t}(x_n)]^\top$ and  $\vec{y} = [y_1, \dots, y_n]^\top$. Let us call this approach as {\tt Feature-Map-Learning}. 

Here, we empirically compare {\tt Joint-Gradient-Descent} approach and {\tt Feature-Map-Learning} approach. We used 3-layer fully connected neural nets as $\vec{\phi}_\theta$, where it maps input $x$ to 32-dimensional vector. The size of the hidden layer is set to 64. We used MNIST datasets, where $x_i$ is the image and $y_i$ is the label. We used ADAM for gradient-based optimization algorithm. Figure~\ref{fig:feature_map_learning} shows the learning curves of the two approaches. From Figure~\ref{fig:feature_map_learning}, we can see that {\tt Feature-Map-Learning} approach converges faster than {\tt Joint-Gradient-Descent} and reaches to the solution that generalizes well.

\begin{figure}
    \begin{small}
        \begin{center}
            \includegraphics[width=0.95\textwidth]{Appendix/comparison.pdf}
        \end{center}
        \caption{Comparison of two approaches}
        \label{fig:feature_map_learning}
    \end{small}
\end{figure}



==> junk_piece/junk_appendices/hyper-param.tex <==
In this appendix, we introduce the way of tuning the hyper-parameter $\lambda_1, \lambda_2$. In KIV, this is done by optimizing the stage 1 and stage 2 error evaluated by the out-of-sample. This approach, however, is not valid in DFIV since we alternatively update stage 1 model and stage 2 model. Instead, we propose to choose hyper-parameter jointly from the out-of-sample stage 2 loss. Formally, let denote complete stage 1 data as $(x_i, y_i, z_i)$, and $\lambda_1, \lambda_2$ is chosen that minimizes
\begin{align*}
    \hat{\mathcal{L}}_2^{(\mathrm{oos})} = \frac{1}{m} \sum_{i=1}^m \|y_i - (\hat{\vec{f}}^{(n)})^\top \hat{E}^{(m)} \vec{\phi}_{\theta_Z}(z_i)\|^2.
\end{align*}
Note that $\hat{E}^{(m)}$ and $\hat{\vec{f}}^{(n)}$ are the solution of stage 1 and 2, respectively.


==> junk_piece/junk_appendices/proof-thm-1.tex <==
Here, we prove Theorem~\ref{thm:approximation}, which states that our simple kernel function can express the complex function.

\begin{proof}
    Let $\kappa$ be a shift-invariant kernel function on $[0,1]^d$. From Claim 1 in \citet{Rahimi2008}, there exists a random algorithm that generates random matrix $A \in \mathbb{R}^{D\times d}$ and vector $\vec{b} \in \mathbb{D}$ such that
    \begin{align*}
        \prob{\sup_{\vec{x}, \vec{y}}\|(\cos(A\vec{x} + \vec{b}))^\top(\cos(A\vec{y} + \vec{b})) - \kappa(\vec{x}, \vec{y})\|^2 \geq \varepsilon} \leq 2^8 \frac{\sigma_p^2 d}{\varepsilon^2}\exp\left(-\frac{D\varepsilon^2}{4(d+2)}\right),
    \end{align*}
    where $\sigma_p$ is a constant depending on $\kappa$ and cosine function is appled element-wise $\cos(\vec{x}) = (\cos(x_1), \cos(x_2), \dots)^\top$. From the inequality above, we can see that the probability is strictly less than 1 if we set $D = \Omega(\frac{d}{\varepsilon^2}\log\frac{d}{\varepsilon})$. Hence, we can conclude that there exists $\tilde A, \tilde{\vec{b}}$ such that 
    \begin{align*}
        \sup_{\vec{x}, \vec{y}}\|(\cos(\tilde A\vec{x} + \tilde{\vec{b}}))^\top(\cos(\tilde A\vec{y} + \tilde{\vec{b}})) - \kappa(\vec{x}, \vec{y})\|^2 \leq \varepsilon
    \end{align*}
    from the probablistic method \citep{alon04}. Therefore, the $L+1$-layer network  $\tilde\psi(\vec{x}) = \cos(\tilde A\vec{x} + \tilde{\vec{b}})$ satisfies the condition given in the theorem.
\end{proof}

==> junk_piece/junk_appendices/test_points.tex <==
Figure~\ref{fig:testpoints} shows plot of $(p,t)$ appears in train time and test time.
the train points and test points in the demand design problem. From Figure~\ref{fig:testpoints}, we can see that the model is required to predict the points where no training point exists. In other words, the model needs to extrapolate the prediction in order to achieve a good performance in this experiment.

\begin{figure}[H]
    \begin{small}
        \begin{center}
            \includegraphics[width=0.7\textwidth]{Appendix/testpoints.pdf}
        \end{center}
        \caption{train points and test points of price $p$ and time of the year $t$}
        \label{fig:testpoints}
    \end{small}
\end{figure}

Such change of distribution damages the vanilla DFIV, which Spectral Normalization is not applied. Figure~\ref{fig:fail} shows the 200 test points with the largest prediction error.

\begin{figure}[H]
    \begin{small}
        \begin{center}
            \includegraphics[width=0.7\textwidth]{Appendix/failing.pdf}
        \end{center}
        \caption{200 test points that vanilla DFIV fails}
        \label{fig:fail}
    \end{small}
\end{figure}

From Figure~\ref{fig:fail}, we can see that the vanilla DFIV fails at the test points where there is little training points around.
To deal with this problem, we need to make have to impose smoothness on the model we learn. This is the reason why this setting is favorable for KIV\citep{Singh2019} method, which uses the prespecified smooth feature maps. DeepIV\citep{Hartford2017} also implicitly regularizes the model by stochastically perturbing the input to Stage 2 regression problem according to the conditional distribution estimated in Stage 1 regression.

==> junk_piece/junk_appendices/z_tuning.tex <==
One might want to jointly minimize the loss $\tilde{\mathcal{L}}^{(n)}_2$, which is the empirical approximation of $\mathcal{L}$. However, this fails to learn true structural function $f_{\mathrm{str}}$, as shown in this appendix.

Figure~\ref{fig:learning_fail} shows the learning curve when we jointly minimize $\theta_X$ and $\theta_Z$ with respect to $\tilde{\mathcal{L}}^{(n)}_2$, where $\mathcal{L}_{\mathrm{test}}$ is the empirical approximation of
\begin{align}
    {L}_{\mathrm{test}} = \expect[X]{\|f_{\mathrm{text}}(X) - (\hat{\vec{f}}^{(n)})^\top\vec{\psi}_{\theta_X}(X)\|^2}.
\end{align}

\begin{figure}
    \begin{small}
        \begin{center}
            \includegraphics[width=0.95\textwidth]{Appendix/learning_curve_fail.pdf}
        \end{center}
        \caption{Learning curve of joint minimization}
        \label{fig:learning_fail}
    \end{small}
\end{figure}

From Figure~\ref{fig:learning_fail}, we can see that the decrease of stage 2 loss does not improve the performance of the learned structural function. This is because the model focuses on learning the relationship between instrument $Z$ and outcome $Y$, while ignoring treatment $X$. We can see this from the fact that stage 1 loss becomes large and unstable. This is against the goal of IV regression, which is to learn a good causal relationship between $X$ and $Y$.

On the other hand, Figure~\ref{fig:learning_suc} shows the learning curve of the DFIV. Now, we can see that stage 2 loss matches $\mathcal{L}_{\mathrm{test}}$. Also, we can confirm that stage 1 loss stays small and stable.

\begin{figure}
    \begin{small}
        \begin{center}
            \includegraphics[width=0.95\textwidth]{Appendix/learning_curve_suc.pdf}
        \end{center}
        \caption{Learning curve of DFIV}
        \label{fig:learning_suc}
    \end{small}
\end{figure}


==> junk_piece/kiv.tex <==
In KIV, structural function $f$ is searched in a RKHS. Let $k_\mathcal{X}:\mathcal{X} \times \mathcal{X} \to \mathbb{R}$ and $k_\mathcal{Z}:\mathcal{Z} \times \mathcal{Z} \to \mathbb{R}$ be the positive semi-definite kernels, and $\mathcal{H}_\mathcal{X}, \mathcal{H}_\mathcal{Z}$ be the RKHS induced by $k_\mathcal{X}$ and $k_\mathcal{Z}$, respectively. We denote the feature map to these spaces as $\psi(x) = k_\mathcal{X}(x,\cdot)$ and  $\phi(z) = k_\mathcal{Z}(z,\cdot)$. If we consider the minimization in $f \in \mathcal{H}_\mathcal{X}$ and use Tikhonov regularization $\Omega(f) = \lambda_1\|f\|^2_{\mathcal{H}_\mathcal{X}}$, from the characteristics of reprodusing kernel, loss in \eqref{eq:total-loss} becomes
\begin{align*}
    \mathcal{L}(f) = \expect[YZ]{(Y - \braket[{\mathcal{H}_\mathcal{X}}]{f, \mu_{X|Z}})^2} + \lambda_1\|f\|^2_{\mathcal{H}_\mathcal{X}}, 
\end{align*} 
where $\mu_{X|Z}$ is a conditional mean embedding defined as $\mu_{X|z} = \expect{\phi(X) | z}$. As discussed previously, the goal of stage 1 is to obtain the estimation of the conditional expectation $\expect[X|z]{f(X)}$, hence it is sufficient to consider the conditional mean operator $E$ that maps $\phi(z)$ to $\mu_{X|z}$. Such operator can be learned from the following minimization.
\begin{align}
    \hat{E} = \argmin_{E: \mathcal{H}_\mathcal{Z} \to \mathcal{H}_\mathcal{X}} \mathcal{L}_1(E), \quad
    \mathcal{L}_1(E) = \expect[X,Z]{\|\psi(X) - E \phi(Z)\|_{\mathcal{H}_\mathcal{X}}} + \lambda_1 \|E\|_{\mathcal{H}_\mathcal{Z} \to \mathcal{H}_\mathcal{X}}^2. \label{eq:stage1-loss}
\end{align}
In stage 2, we find $f$ by minimizing loss $\mathcal{L}(f)$ with the conditional expectation is replaced by the estimation in stage 1.
\begin{align}
    \hat{f} = \argmin_{f\in\mathcal{H}_\mathcal{X}} \mathcal{L}_2(f)\quad \mathcal{L}_2(f) = \expect[Y,Z]{(Y -  \braket[{\mathcal{H}_\mathcal{X}}]{f, \hat{E}\phi(Z)})^2}. \label{eq:stage2-loss}
\end{align}

Thanks to reproducing characteristics, minimization in \eqref{eq:stage1-loss} and \eqref{eq:stage2-loss} can be solved analytically. In this work, we propose the method to use adaptive feature maps that further reduce the loss.



==> junk_piece/low_dim.tex <==
In this low dimenonal case, we consider  treatment variable $X$ to be $X = (p,t,s)$ and instrumental variable $Z$ to be $Z = (c,t,s)$, which is the standard benchmark for IV regression problem. We compare our DFIV method to two leading competitors, namely  KIV \citep{Singh2019} and DeepIV \citep{Hartford2017}.

In the experiment, we used the same network architecture for feature map $\vec{\psi}_{\theta_X}, \vec{\phi}_{\theta_Z}$ as DeepIV. We tune the regularizer $\lambda_1,\lambda_2$ in the way discussed in Appendix~\ref{sec:hyper}, and the data is evenly split for stage 1 and stage 2. To cope with the extrapolation problem, we apply Spectral Normalization \citep{Miyato2018} during the learning to enhance the smoothness of feature maps.
 

 We test the case where the total datasize is $n+m=\{1000, 5000, 10000\}$. For each algorithm and sample size, we ran 20 simulations.  The result is summarized in Figure~\ref{fig:demand}, where {\tt DFIV(vanilla)} presents the performance of DFIV without applying Spectral Normalization.
 
\begin{figure}[t]
    \begin{small}
        \begin{center}
            \includegraphics[width=1.0\textwidth]{Experiment/demand.pdf}
        \end{center}
        \caption{MSE for Demand design dataset with low dimensional confounders.}
        \label{fig:demand}
    \end{small}
\end{figure}

DFIV and DeepIV exhibit similar performance when we have enough amount of data, though DFIV performs significantly better than DeepIV when the data size is small. Moreover, the variances of MSE of DFIV tend to be smaller than that of DeepIV. Considering that these two methods share the same network architecture, this suggests that the learning methodology of DFIV is more stable and sample-efficient compared to DeepIV. Moreover, although the setting is more favorable for KIV, since it is designed to learn a extrapolatable smooth structural function, DFIV can match its performance when Spectral Normalization is applied.

==> junk_piece/rff_part.tex <==

Although \eqref{eq:kernel-def} is the simplest form of the deep kernel, we claim that it does not sacrifice the expressiveness of the deep kernel. One way of seeing this is to consider the random Fourier feature \citep{Rahimi2008}.

\begin{thm}\label{thm:approximation}
    Given deep kernel function $k(x, x') = \kappa(\psi(x), \psi(x'))$ where $\kappa$ is the shift-invariant kernel function and $\psi(x')$ is a $L$-layer neural network whose output is bounded to $[0,1]^d$. Then, with an arbitrarily small $\varepsilon >0$, there exists $(L+1)$-layer neural network $\tilde{\psi}(x)$ with $D$-dimensional output that satisfies
    \begin{align*}
        \sup_{x, x'} |k(x, x') - (\tilde{\psi}(x))^\top (\tilde{\psi}(x'))|  \leq  \varepsilon     
    \end{align*}
    when $D = \Omega(\frac{d}{\varepsilon^2} \log \frac{d}{\varepsilon})$ and the cosine activation function is used in the final layer.
\end{thm}

The proof is based on the probabilistic method \citep{alon04} and \citep[Claim~1]{Rahimi2008} and given in Appendix~\ref{sec:proof}. Theorem~\ref{thm:approximation} suggests that our kernel is not less expressive compared to more complex deep kernels. In practice, we might not use cosine activation function, though we can still approximate complex deep kernel by simply adding extra layers. Considering that most popular kernel functions, such as RBF kernel and Matern kernel \citep{Rasmussen2005}, are shift-invariant, we suppose the expressive power of our simple deep kernel is comparable to more complex deep kernel functions.


==> junk_piece/scalability.tex <==
The computational complexity of the proposed algorithm is $O(md_1d_2 + d_2^3)$ at stage 1, while stage 2 requires additional $O(nd_1d_2 + d_1^3)$ computations. This is small compared to the KIV method \citep{Singh2019}, which takes $O(m^3)$ and $O(n^3)$, respectively, and due to the fact that we are using using the inner product deep kernel \eqref{eq:kernel-def}. The computational bottleneck of the KIV method is to compute the inverse of Gram matrix $K=(k(z_i, z_j))_{i,j}$, which is inevitable if we use infinite-dimensional feature map. However, by using a finite-dimensional feature map, our formulation avoids a costly matrix inversion. 

Our method is also substantially faster than DeepIV method \citep{Hartford2017}, although both computational complexities are linear in the data size. In DeepIV, we need to estimate the density of conditional distribution $\expect[X|z]{\vec{\psi}(X)}$\adcomment{$P(X | Z)$}, which is unstable and difficult to parallelize\adcomment{substantiate better this claim, reference?}. On the other hand, the losses $\tilde{\mathcal{L}}_1^{(m)}, \tilde{\mathcal{L}}_2^{(n)}$ in DFIV methods only require us to perform matrix multiplications, which is stable and easy to parallelize.

==> junk_piece/stage2_old.tex <==
As in stage 1, we can update $\theta_X$ based on loss $\tilde{\mathcal{L}}^{(n)}_2$ defined as
\begin{align*}
    \tilde{\mathcal{L}}^{(n)}_2 &= \frac1n \sum_{i=1}^n (\tilde y_i -(\hat{\vec{f}}^{(n)})^\top \hat{E}^{(m)} \vec{\phi}_{\theta_Z}(\tilde z_i))^2 + \lambda_2 \|\vec{f}^{(n)}\|^2\\
    %&= \frac1n \|\vec{y}\|^2 -\frac1n \vec{y}^\top \Phi_2(\hat{E}^{(m)})^\top \left(\hat{E}^{(m)}\Phi_2 ^\top \Phi_2 (\hat{E}^{(m)})^\top + n\lambda_2 I\right)^{-1}\hat{E}^{(m)}\Phi_2^\top \vec{y}\\
    &= \frac1n \|\vec{y}_2\|^2 - \frac1n \vec{y}_2^\top A \Psi_1(\Psi^\top_1 A^\top A \Psi_1 + n\lambda_2 I)^{-1} \Psi_1^\top A^\top \vec{y}_2,
\end{align*}
where $A = \Phi_2(\Phi_1^\top \Phi_1 + \lambda_1I)^{-1}\Phi_1^\top \in \mathbb{R}^{n\times m}$. The second equation holds from the definition of $\hat{f}^{(n)}$ and $\hat{E}^{(m)}$ given in \eqref{eq:stage1-sol} and \eqref{eq:stage2-sol}, respectively. Recall that $\Psi_1$ is a feature matrix of treatment variable $X$, which explicitly depends on $\theta_X$. Therefore, we can update $\theta_X$ based on the gradient of $\tilde{\mathcal{L}}_2^{(n)}$, which can be computed by off-the-shelf auto-differentiation libraries.
 
One might attempt to tune $\theta_Z$ as well to minimize the $\tilde{\mathcal{L}}_2^{(m)}$. However, this is inappropriate since the goal of IV regression is not to regress $Z$ instrumental variable to $Y$. In experiments, we observed that if we tune $\theta_Z$ in stage 2, we could achieve the lower value of loss $\tilde{\mathcal{L}}^{(m)}_2$, while the structural function learned separately.\adcomment{i am not sure what you are trying to say here, only made sense after reading appendix and looking at Figure 7}

